Structure-Blind Signal Recovery

We consider the problem of recovering a signal observed in Gaussian noise. If the set of signals is convex and compact, and can be specified beforehand, one can use classical linear estimators that achieve a risk within a constant factor of the minimax risk. However, when the set is unspecified, designing an estimator that is blind to the hidden structure of the signal remains a challenging problem. We propose a new family of estimators to recover signals observed in Gaussian noise. Instead of specifying the set where the signal lives, we assume the existence of a well-performing linear estimator. Proposed estimators enjoy exact oracle inequalities and can be efficiently computed through convex optimization. We present several numerical illustrations that show the potential of the approach.

==> macros.tex <==
\def\cR{\Re}
\def\cC{{\cal C}}
\def\Risk{\mathop{\hbox{\rm Risk}}}
\newcommand{\half}{ \mbox{\small$\frac{1}{2}$}}
\newcommand{\four}{ \mbox{\small$\frac{1}{4}$}}
\def\Opt{{\hbox{Opt}}}
\def\dist{{\hbox{dist}}}
\def\bR{{\mathbf{R}}}
\def\bZ{{\mathbf{Z}}}
\def\Cov{{\hbox{\rm Cov}}}
\def\ErfInv{\mathop{\hbox{\rm ErfInv}}}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}[1]{\label{#1}\end{eqnarray}}
\newcommand{\nn}{\nonumber \\}
\newcommand{\ese}{\end{eqnarray*}}
\newcommand{\bse}{\begin{eqnarray*}}
\newcommand{\rf}[1]{~(\ref{#1})}
\def\qed{\hfill$\square$}
\def\cP{{\cal P}}
\def\cG{{\cal G}}
\def\cQ{{\cal Q}}
\def\cB{{\cal B}}
\def\cX{{\cal X}}
\def\cS{{\cal S}}
\def\cU{{\cal U}}
\def\cR{{\cal R}}
\def\cT{{\cal T}}
\def\cJ{{\cal J}}
\def\cM{{\cal M}}
\def\cO{{\cal O}}
\def\cI{{\cal I}}
\def\cJ{{\cal J}}
\def\reg{{\hbox{\scriptsize\rm con}}}
%\def\lasso{{\hbox{\scriptsize\rm lasso}}}
\def\lasso{{\hbox{\scriptsize\rm pen}}}
\def\pen{{\hbox{\scriptsize\rm pen}}}
\def\Erf{\mathop{\hbox{\rm Erf}}}
\def\Conv{\mathop{\hbox{\rm Conv}}}
\def\Tr{\mathop{\hbox{\rm Tr}}}
\def\cZ{{\cal Z}}
\def\cl{\mathop{\hbox{\rm cl}}}
\def\Ker{\mathop{\hbox{\rm Ker}}}
\def\argmin{\mathop{\hbox{\rm argmin}}}
\def\bK{{\mathbf{K}}}
\def\bS{{\mathbf{S}}}
\def\conv{{\hbox{Con}}}
\def\Lin{{\hbox{\rm Line}}}
\def\cbl{\color{blue}}
\def\Diag{{\hbox{\rm Diag}}}
\def\CVaR{{\hbox{\rm CV@R}}}
\def\mones{{\mathbf{e}}}
\def\E{{\mathbf{E}}}
\def\cA{{\cal A}}
\def\N{{\mathcal{N}}}
\def\CN{{\C\mathcal{N}}}
\def\S{{\mathcal{S}}}
\def\F{{\mathcal{F}}}
\def\H{{\mathcal{H}}}
%\def\E{\mathbbm{E}}
\def\C{\mathbb{C}}
\def\R{\mathbb{R}}
\def\Z{\mathbb{Z}}
\def\Prob{{\hbox{\rm Prob}}}
\def\e{{\rm e}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\def\Argmax{\mathop{\hbox{\rm Argmax}}}
\def\Argmin{\mathop{\hbox{\rm Argmin}}}
%\newcommand{\subsubsubsection}[1]{\bigskip\par\noindent{\bf #1}\medskip\par\noindent}
\def\Card{\mathop{\hbox{\rm Card}}}
\def\Risk{\hbox{\rm Risk}}
\def\ccy{\color{cyan}}
\def\crd{\color{red}}
\newcommand{\cz}[2]{{\color{blue}#2}}
\newcommand{\ci}[2]{{\color{blue}#2}}
\newcommand{\dimacorr}[2]{{\color{magenta}#2}}
\newcommand{\mynote}[1]{{\bf \color{red}{#1} }\\}
\newcommand{\prob}{\text{Prob}}
\newcommand{\flasso}{F-lasso} 
